Frequency-hiding Dependency-preserving Encryption for Outsourced Databases

The cloud paradigm enables users to outsource their data to computationally powerful third-party service providers for data management. Many data management tasks rely on the data dependencies in the outsourced data. This raises an important issue of how the data owner can protect the sensitive information in the outsourced data while preserving the data dependencies. In this paper, we consider functional dependency FD, an important type of data dependency. We design a FD-preserving encryption scheme, named F2, that enables the service provider to discover the FDs from the encrypted dataset. We consider the frequency analysis attack, and show that the F2 encryption scheme can defend against the attack under Kerckhoff's principle with provable guarantee. Our empirical study demonstrates the efficiency and effectiveness of F2.

==> encryptionmethod.tex <==
\section{Data Encryption Scheme}

One of the most important questions for cleaning of inconsistent data is how to model the consistency of the data, i.e., how to specify and determine that the data is clean? 
Recent work specifies the consistency of data in terms of integrity constraints, and detects inconsistencies in the data as violations of the constraints \cite{arenas1999consistent,chomicki2005minimal,franconi2001census,wijsen2002condensed}. A variety of formalisms have recently been studied to specify integrity constraints as data quality rules, including 
functional dependencies (FDs) \cite{huhtala1999tane}, conditional functional dependencies (CFDs) \cite{chiang2008discovering, golab2008generating,DBLP:journals/tkde/FanGLX11,DBLP:conf/icde/FanGLX09}, order dependencies (ODs) \cite{ginsburg1983order,ng1999ordered}, currency dependencies (CDs) \cite{fan2012determining}, sequential dependencies (SDs) \cite{golab2009sequential}, matching dependencies (MDs) \cite{fan2009reasoning,fan2011dynamic}, editing rules (eRs) \cite{fan2010towards}, denial constraints \cite{arenas1999consistent,chomicki2005minimal}, and inclusion dependencies (INDs) \cite{arenas1999consistent}.  In this paper, we consider FDs as the integrity constraints that are to be enforced for data consistency. 
Formally, given a relation $R$, a set of attributes $Y$ in $R$ is said to be {\em functionally dependent} on another set of attributes $X$ in $R$ (denoted $X\rightarrow Y$) if and only if for any pair of tuples $r_1, r_2$ in $R$, if $r_1[X] =r_2[X]$, then $r_1[Y]=r_2[Y]$. 

An essential step of identifying and fixing inconsistent data is to find the integrity constraints of the data. It is often unrealistic to rely solely on human experts to design data quality rules via expensive manual process.  Therefore, it is necessary to have techniques that can automatically discover integrity constraints from the data. Our goal is to design data transformation schemes on the outsourced datasets that enable the service provider to: (1) discover FDs from the outsourced (encoded) dataset automatically, and (2) suggest the repair of inconsistent data based on the discovered integrity constraints. 

There are three requirements of the encryption scheme:
\begin{itemize}
\item {\em One-to-many substitution}: This substitution can defend against the frequency analysis attack.
\item {\em FD-preserving}: the FDs of the original datasets must hold in the encrypted dataset.
\item {\em Repairable inconsistency}: The inconsistent data in the encrypted data should still be repairable. 
\end{itemize}

\subsection{One-to-many FD-preserving Substitution Encryption}
\input{encryption}

\nop{
\subsection{FD-preserving Encryption}

Simply applying the one-to-many substitution in our previous work \cite{wang2006efficient} to the $DCaS$ paradigm may destroy the FDs. For instance, assume the dataset has the FD $X\rightarrow Y$. By our one-to-many substitution scheme \cite{wang2006efficient}, the tuples that contain ($X=x_1, Y=y_1$) pair will be encrypted as ($X=E_{x_1}^1, Y=E_{y_1}^1$) and ($X=E_{x_1}^1, Y=E_{y_1}^2$). Apparently, the FD $X\rightarrow Y$ does not hold anymore. Therefore, we propose to design  {\em FD-preserving one-to-many substitution cipher scheme} that 
is built around the notion {\em equivalent classes} \cite{bohannon2005cost}. The semantics of an equivalent class of any pair $(t, A)$, where $t$ is a tuple and $A$ is a set of attribute, is that the tuple attributes contained in the class are assigned the same value in the dataset. 
This requires that the one-to-many substitution cipher schemes indeed construct equivalent classes for the data pairs across all attributes that are involved in any FD.  
This is extremely challenging given the fact that the client is not aware of any FD when she designs and applies the encoding scheme. Furthermore, the fact that multiple FDs possibly overlap will add additional layer of complexity to this problem. 
We will explore novel solutions to the design of FD-preserving one-to-many substitution cipher schemes. Our preliminary solution is to apply one-to-many substitution scheme at the granularity of a set of attributes \{$X_1, \dots, X_t$\}, instead of on every single attribute. Then if the attributes \{$X_1, \dots, X_t$\} cover all attributes in the FDs, the substitution scheme must be FD-preserving. 

{\bf Unsolved technical issues.} First, it is challenging to pick the appropriate $t$ value that decides the number of attributes involved in the substitution cipher. Large $t$ values ($t$ equals to the total number of attributes for the worst case) may be too restrict, while small $t$ values may miss some FDs (e.g., only considering $t=2$ may fail to preserve any FD that involves more than two attributes). Second, FDs may overlap at some attributes (e.g., $A\rightarrow B$ and $A\rightarrow C$). Then any substitution cipher scheme that  considers attribute pairs independently may fail to deliver the data that satisfies multiple FDs that overlap. Third, it is not guaranteed that the cipher values constructed by the FD-preserving one-to-many substitution cipher still behave the  uniform distribution at each attribute (and thus can defend against the frequency analysis attack). 
 
\subsection{Inconsistency-repairable Encryption}
There is often a very large number of ways to modify a table to make it satisfy all the required FDs \cite{beskales2010sampling}. 
One way is to delete all tuples that violate FDs \cite{chomicki2005minimal,chomicki2004computing} or modify the attribute values that violate FDs \cite{bohannon2005cost}. Another approach computes answer  
to selected classes of queries that are valid in every possible 
``reasonable'' repair \cite{arenas1999consistent,chomicki2004computing,chomicki2005minimal,fuxman2005first,wijsen2002condensed,wijsen2005database}. In this project, we mainly focus on the first repair approach that modifies the data to make it consistent with the discovered FD constraints. We will investigate the feasibility of applying the existing FD discovery algorithms (e.g., \cite{huhtala1999tane}) on the encoded data. 
The privacy-preserving data repair mechanism is seemly straightforward from the FD-preserving substitution cipher scheme; any existing FD repair algorithm (e.g., \cite{bohannon2005cost}) can be applied to the encrypted data to fix the inconsistency if the encrypted data has preserved FDs. However, this is indeed not true. 
Consider a dataset $D$ that has a FD $F: X\rightarrow Y$. Assume the $(X=x_1, Y=y_1)$ pair is encrypted as $(X=E_{x_1}^1, Y=E_{y_1}^1)$ and $(X=E_{x_1}^2, Y=E_{y_1}^2)$ by our FD-preserving one-to-many substitution scheme (Task 2.A.1). Now assume $D$ contains a record that contains the data pair $(X=x_1, Y=y_2)$, which is inconsistent with the FD $F$. Assume $(X=x_1, Y=y_2)$ is encrypted to $(X=E_{x_1}^3, Y=E_{y_2}^1)$ and $(X=E_{x_1}^4, Y=E_{y_2}^2)$ by our FD-preserving one-to-many substitution cipher scheme. Now $(X=E_{x_1}^3, Y=E_{y_2}^1)$ and $(X=E_{x_1}^4, Y=E_{y_2}^2)$ cannot be identified as inconsistent by the server as it is not aware that $E_{x_1}^3$ and $E_{x_1}^4$ are indeed mapped to the same plaintext value. Indeed, allowing the server to know that both $E_{x_1}^3$ and $E_{x_1}^4$ are mapped to $x_1$ will bring privacy vulnerabilities by a sophisticated frequency analysis. To address the dilemma, we will consider {\em approximate FDs} \cite{bohannon2005cost} instead of exact $FDs$. It has been shown in the literature that due to the existence of inconsistent data, the data repair procedure should rely on {\em approximate FDs} \cite{bohannon2005cost} instead of exact ones. Formally, the error $e(F)$ of a dependency $F: X\rightarrow Y$ is defined as the minimum number of tuples that need to be removed from the given dataset $D$ to make $X\rightarrow Y$ holds in $D$. 
The approximateness of a dependency $F: X\rightarrow Y$ is defined as $\frac{e(F)}{|D|}$, the fraction of tuples of $D$ that contribute to the error of $F$. Given an error threshold $\epsilon\ (0\leq\epsilon\leq 1)$, we say a function $F$ is an {\em approximate FD} if its approximateness is no larger than $\epsilon$. We believe that the  $\epsilon$ value should be valued based on the reasoning of our FD-preserving one-to-many substitution cipher scheme. Intuitively, mapping to more ciphertext values requires a higher $\epsilon$ value. We will investigate the details and complete the design of our privacy-preserving repair algorithms. 
}
